Ctrl-V: Higher Fidelity Video Generation with Bounding-Box Controlled Object Motion

Controllable video generation has attracted significant attention, largely due to advances in video diffusion models. In domains such as autonomous driving, it is essential to develop highly accurate predictions for object motions. This paper tackles a crucial challenge of how to exert precise control over object motion for realistic video synthesis. To accomplish this, we 1) control object movements using bounding boxes and extend this control to the renderings of 2D or 3D boxes in pixel space, 2) employ a distinct, specialized model to forecast the trajectories of object bounding boxes based on their previous and, if desired, future positions, and 3) adapt and enhance a separate video diffusion network to create video content based on these high quality trajectory forecasts. Our method, Ctrl-V, leverages modified and fine-tuned Stable Video Diffusion (SVD) models to solve both trajectory and video generation. Extensive experiments conducted on the KITTI, Virtual-KITTI 2, BDD100k, and nuScenes datasets validate the effectiveness of our approach in producing realistic and controllable video generation.

==> sections/abstract_arxiv.tex <==
\begin{abstract}
With recent advances in video prediction, controllable video generation has been attracting more attention. Generating high fidelity videos according to simple and flexible conditioning is of particular interest. To this end, we propose a controllable video generation model using pixel level renderings of 2D or 3D bounding boxes as conditioning. In addition, we also create a bounding box predictor that, given the initial and ending frames' bounding boxes, can predict up to 15 bounding boxes per frame for all the frames in a 25-frame clip.  We perform experiments across 3 well-known AV video datasets: KITTI, Virtual-KITTI 2 and BDD100k.\\
\textbf{Project page: \url{https://oooolga.github.io/ctrl-v.github.io/}}.
\end{abstract}

% \keywords{Video Generation, Stable Video Diffusion, ControlNet, Motion Control} 

==> sections/method_old.tex <==
In this section, we outline our simple yet robust method for creating video clips that strictly adhere to specified frame-level bounding-box guidelines. Ctrl-V encompasses two closely related sub-models: 1) \modelbbox~(Section~\ref{sec:bbox_predictor}): a modified Video Latent Diffusion Model (VLDM) to generate bounding-box frames, images of only bounding boxes; 2) \modelvid (Section~\ref{sec:controlnet}): our video generation model that allows precise frame-level conditioning. The overall model diagram is shown in Figure~\ref{fig:model_diagram}. In the following, we provide a brief overview of the preliminaries before delving into the details of Ctrl-V.
\subsection{Preliminaries}\label{sec:svd_intro}
% \textit{To clarify terminology and prevent confusion due to the varying timesteps used in the diffusion denoising process and video sequences, our mathematical formulation will employ subscript indices to denote the denoising timestep, and superscript indices to represent the frame index within a video sequence.}

Stable Video Diffusion (SVD) \citep{blattmann2023stable, blattmann2023align} is a cutting-edge video generation model that excels in converting still images into dynamic video sequences. The pretrained SVD model employed in this project has been pretrained using the Euler discrete noise scheduling method outlined by \citet{karras2022elucidating}. The objective of the SVD model is to generate a video sequence \(\vf = [\vf^{(0)}, \ldots, \vf^{(N)}]\) starting from an initial frame \(\vf^{(0)}\), where \(K\) represents the sequence length. 


The SVD model utilizes an image autoencoder to encode and decode each frame, converting them between pixel space and latent space. Mathematically, this process is represented as \( \De\big(\En(\vf)\big) = \De(\vz)\approx \vf \), where \(\En\) is the image encoder, \(\De\) is the image decoder and \(\vz\) is the latent space representation of frame \(\vf\). In SVD, the diffusion process occurs within the latent space. This process entails gradually introducing noise to the latent representations. Subsequently, the denoiser network is responsible for removing this added noise from the noisy latent representations. The denoiser network \(\sD_\theta\), trained under the Euler discrete noise scheduling schema, can be described by the formulation:
\begin{equation}
    \sD_\theta(\vz; \sigma_t)=\lambda_{\text{skip}}(\sigma_t)\vz + \lambda_\text{out}(\sigma_t)\sU_\theta\big(\lambda_\text{in}(\sigma_t)\vz, \vz^{(0)}_{\text{pad}}, \vc^{(0)}; \lambda_\text{noise}(\sigma_t)\big)
    \label{eq:denoiser}
\end{equation}
Here \(\lambda_{\text{skip}}\), \(\lambda_{\text{out}}\), \(\lambda_{\text{in}}\) and \(\lambda_{\text{noise}}\) are scaling functions and \(\sigma_t\) is the computed noise level at time $t$; the mathematical definitions of these terms are detailed in Appendix~\ref{sec:svd_notation}. \(\sU_\theta\) represents the 3D U-Net \citep{ronneberger2015unet}, whose parameters \(\theta\) are optimized for the denoising task during training.

To gain a clearer understanding of the U-Net inputs, we eliminate the scaling terms and reparameterize its input as follows: 
\begin{equation}
    \sU_\theta\big(\hat{\vz}_t, \vz_{\text{pad}}^{(0)}, \vc^{(0)}, t\big)
    \label{eq:unet_input}
\end{equation}
where \(\hat{\vz}_t\in\R^{K\times C'\times H'\times W'}\) denotes the latent representation of frames corrupted by noise at the current noise level \(t\); \(\vz^{(0)}\in\R^{1\times C'\times H'\times W'}\) represents the latent representation of the initial frame, and \(\vc^{(0)}\) represents the encoding of the initial frame image token using CLIP \citep{radford2021clip}. These parameters are introduced into the U-Net through distinct layers. Initially, at the input layer, \(\vz^{(0)}\) undergoes repeated padding along the frame's time dimension to match the dimensions of the \(\hat{\vz}_t\) tensor, namely \(\vz_{\text{pad}}^{(0)}\). Subsequently, the \(\vz_{\text{pad}}^{(0)}\) is concatenated with \(\hat{\vz}_t\) along the channel dimension and passed into the network's input layer. Meanwhile, the noise level indicator \(t\) is transformed into a time-step embedding vector and is subsequently fed into each U-Net block along with \(\vc^{(0)}\) via cross-attention conditioning mechanism \citep{rombach2022highresolution}.

\subsection{Preprocessing: Bounding-Box Rendering}\label{sec:bbox_preprocess}

Bounding boxes can be represented in many ways to be used as input to a network. While work such as Boximator \cite{wang2024boximator} represents bounding boxes as a Fourier transformed concatenated vector of its coordinate, ID and other information,
we choose to create an information-rich image rendering of the bounding boxes as representation. By utilizing different pattern and colors, we are able to encode meta information -- in addition to the location of the bounding boxes -- such as track ID, object types, orientation about every bounding box in each frame; furthermore, by using an image representation, we take advantage of the SVD model's ability to interpret image data without the need to introduce customized adapter.
% We create a method to make bounding-box videos which have significant benefits.
% These videos not only show the precise locations of objects within a scene but also effectively display different kinds of information, like track IDs and object types, using different shapes and colors. 
We also implement a method to render trajectory frames, similar to the bounding-box frames, but without drawing out the entire box. These trajectory frames only contain mid-point location information. The procedure for creating bounding-box/trajectory plots is detailed in Appendix~\ref{sec:bbox_plot_procedure}. 
These bounding-box frames are ultimately sent to an off-the-shelf VAE image-encoder (\(\En\)) to be encoded (the encoder's performance is discussed in Appendix~\ref{sec:bbox_plots}). 
\begin{figure}[h]
    \centering
\includegraphics[width=\textwidth]{figures/CtrlV_model_diagram.png}
    % \caption{The overview of Ctrl-V: (left)~\modelbbox~and (right)~\modelvid.}
    \caption{The diagram illustrates two components of \textbf{Ctrl-V}: (left; \emph{\color{SteelBlue}blue}) the\textbf{~\modelbbox~}and (right; \emph{\color{Orchid}purple})\textbf{~\modelvid}. In this diagram, \emph{\color{red}red vectors} represent the latents of bounding box frames, while \emph{\color{DarkTurquoise}teal vectors} represent the latents of video frames. \emph{Darker colored vectors} indicate latents that are contaminated by noise. The \emph{trapezoidal shapes} in the diagram represent the UNet architecture, with the inverted trapezoids corresponding to the encoder and decoder modules of the UNet. For both models, we use a \textbf{frozen, off-the-shelf VAE} (represented by the \emph{\color{DarkOrange}orange blocks}) to encode images into latent space and decode them back into pixel space. During training, (1) the\textbf{~\modelbbox~}(Sec.~\ref{sec:bbox_predictor}) learns to denoise the noisy bounding box frame latents (represented by the \emph{\color{DarkRed}dark red vector}), conditioned on the first and last bounding box frame latents (the \emph{\color{red}red vectors}) and the padded initial frame latent (the \emph{\color{DarkTurquoise}teal vector}) and (2) the\textbf{~\modelvid~}(Sec.~\ref{sec:controlnet}) denoises the target frame latents (represented by the \emph{\color{DarkCyan}darker teal vector}) by conditioning on the initial frame's latent (\emph{\color{DarkTurquoise}teal vector}; input to the UNet) and the bounding box frame latents (\emph{\color{red}red vectors}; input to the ControlNet). 
The input tensor dimensions in this figure adhere to the notations defined in Sec.~\ref{sec:method}, where \(B\) denotes the batch size, 
\(K\) the frame count, \(C\) the channel size, \(H\) the frame height, and \(W\) the frame width. The prime (\('\)) symbol indicates the modified shape in the latent space.}
    \label{fig:model_diagram}
\end{figure}

\subsection{Ctrl-V: \modelbbox}\label{sec:bbox_predictor}
Our \modelbbox~(as shown on the left in Figure~\ref{fig:model_diagram}) aims to forecast object positions across intermediate frames, given the initial frame, initial bounding-box frame(s) and the final bounding-box/trajectory frame as references. Our approach involves adjusting the SVD network and leveraging it to generate bounding-box frames. Specifically, we modify the inputs of the U-Net, namely \(\vz_t\), \(\vz_\text{pad}^{(0)}\), and \(\vc^{(0)}\) (refer to Equation \ref{eq:unet_input}), to achieve this objective.

Initially, we pass the bounding-box frames through the image encoder (\(\En\)) to obtain their latent representations, denoted as \(\En(\vf_{\text{bbox}})=\vb\in\R^{K \times C' \times H' \times W'}\). Furthermore, we feed the initial frame into both the image encoder and the CLIP encoder, resulting in \(\vz^{(0)} \in \mathbb{R}^{1 \times C' \times H' \times W'}\) and \(\vc^{(0)}\) respectively.


Similar to the original SVD configuration, we replicate the padding procedure from \(\vz^{(0)} \in \mathbb{R}^{1 \times C' \times H' \times W'}\) to \(\vz^{(0)}_\text{pad} \in \mathbb{R}^{K \times C' \times H' \times W'}\).  In this case, we replace the first and last entries of  \(\vz^{(0)}_\text{pad}\) with \(\vb^{(0)}\) and \(\vb^{(N-1)}\) respectively. Additionally, depending on the desired number of initial bounding-box frames for conditioning, we experiment with substituting different quantities of \(\vz^{(0)}\)  frames with various amounts of bounding-box frames. We use \(\tilde{\vb}\) to denote the modified tensor.

Furthermore, we replaced the \(\hat{\vz}_t\) in Equation~\ref{eq:unet_input} with \(\hat{\vb}_t\), where noise at level \(t\) is incorporated into \(\vb\). The primary objective of the denoiser network is to estimate the amount of noise introduced to \(\vb\).

Overall, the input to the \modelbbox's U-Net is represented as 
\(
    \sU^{\text{bbox}}_\omega\big(\hat{\vb}_t, \tilde{\vb}, \vc^{(0)}, t\big) \label{eq:bbox_predictor_unet}
\).

\subsection{Ctrl-V: \modelvid}\label{sec:controlnet}
Given an initial frame and its corresponding sequence of bounding boxes, our aim is to produce a video clip in which the object positions align with the bounding-box sequence. To achieve this, we introduced \modelvid ~network, where we adapt ControlNet for the SVD framework (as shown on the right in Figure~\ref{fig:model_diagram}). Unlike previous works such as Boximator and TrackDiffusion \citep{wang2024boximator, li2024trackdiffusion}, this motion-control model is trained in a single-stage without requiring additional optimization criteria.

Our \modelvid ~comprises two main components: an SVD and a ControlNet. The input to the SVD model remains consistent with Equation~\ref{eq:unet_input}. Regarding the ControlNet, we utilize the image encoder to encode the bounding-box frames \(\En(\vf_{\text{bbox}})=\vb\in\R^{K, C', H', W'}\). Additionally, we incorporate an adapter layer to preprocess the bounding-box latents before adding them to the frame latents. The inputs to the ControlNet are \(\sC_\xi\big(\vb, \hat{\vz}_t, \vz_{\text{pad}}^{(0)}, \vc^{(0)}, t \big)\).


The architecture of ControlNet closely resembles the contraction and mid-blocks of the SVD’s U-Net architecture, a concept introduced by \citep{zhang2023controlnet}. Additionally, at the start of the training phase, ControlNet's weights are initialized to match those of their mirrored layers. Similar to U-Net, the CLIP encoded token of the initial frame (\(\vc^{(0)}\)) and the time-step embedding are also injected into every block within the ControlNet. Finally, the output from each ControlNet block is added to the residual path within the SVD model after zero-convolution computation.

During training, the weights of the SVD model (\(\theta\)) are frozen, while only the weights in the ControlNet (\(\xi\)) are updated.
